Misinformation is not about Bad Facts: An Analysis of the Production and Consumption of Fringe Content

What if misinformation is not an information problem at all? To understand the role of news publishers in potentially unintentionally propagating misinformation, we examine how far-right and fringe online groups share and leverage established legacy news media articles to advance their narratives. Our findings suggest that online fringe ideologies spread through the use of content that is consensus-based and "factually correct". We found that Australian news publishers with both moderate and far-right political leanings contain comparable levels of information completeness and quality; and furthermore, that far-right Twitter users often share from moderate sources. However, a stark difference emerges when we consider two additional factors: 1) the narrow topic selection of articles by far-right users, suggesting that they cherry pick only news articles that engage with their preexisting worldviews and specific topics of concern, and 2) the difference between moderate and far-right publishers when we examine the writing style of their articles. Furthermore, we can identify users prone to sharing misinformation based on their communication style. These findings have important implications for countering online misinformation, as they highlight the powerful role that personal biases towards specific topics and publishers' writing styles have in amplifying fringe ideologies online.

==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes, see the Ethical Statement.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, see the Datasets and Measures.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see the Conclusion and Discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerYes{Yes, see the Broader Potential Impact of Work.}
    %\answerNo{No, because we are suggesting to utilize }
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, see the Broader Potential Impact of Work.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, see the Data Collection and Management.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{No, we will include our git repository once the paper gets accepted. The repository will include the code and instructions.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{NA. We report accuracy and F1 scores.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{No, the scale of the experiments were small and everything was performed on a PC.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerYes{Yes, see the Online Extreme Groups: misleading styles.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes.}
  \item Did you mention the license of the assets?
    \answerNo{No, the only license we needed was for LIWC and we have the license.}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerYes{Yes.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{NA, we use publicly available datasets and resources.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{NA}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerNA{NA}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{NA}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{NA}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{NA}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{NA}
\end{enumerate}

\end{enumerate}

==> sections/sec1-intro-v1.tex <==
% !TeX root = ../main.tex
%
\section{Introduction}
\label{sec:introduction}

\begin{comment}
\verify{
    I suggest the following changes to the structure:
    \begin{itemize}
        \item Sec 2: section of ``Datasets \& Prerequisites'' (Google News -- remove TDE name --, Twitter far right, Facebook antivax and Facebook far-right) and measures of content (Trust Index) and style (LIWC, StyloMetrix, Grievances)
        \item Sec 3 (or 4): We start by showing there is very little difference between the news articles published by publishers of different political leaning (including far-right). We measure the completeness of the information and even the style. We look at articles produced by publishers considered far-right and those shared by far-right Twitter users. Almost as if the problem is not in the information itself.
        \item Sec 4 (or 3): our main contribution: misinformation and problematic content is an eco-system + styling + personas + qualitative experiment Need here:
        \begin{itemize}
            \item the cards of the personas (maybe in SI)
            \item bring together the identification of style and identification of groups in this order. We need tables of results.
            \item statistical testing results on ads experiment? See \url{https://towardsdatascience.com/a-b-testing-a-complete-guide-to-statistical-testing-e3f1db140499}, section "Discreete metrics"
        \end{itemize}
        \item sec 5: Related work
        \item Sec 6: conclusion
    \end{itemize}
}
\end{comment}

Misinformation can broadly be defined as false and inaccurate narratives that people may believe and communicate despite the existence of a social or expert consensus on the topic. 
% \EB{Can't really say a belief is wrong}
Although not purposefully spread to create harm (which would be called disinformation), misinformation can cause significant societal disruption.
For example, anti-vaccination rhetoric can cause families to withhold vaccination and expose children to life-threatening but preventable diseases such as measles and poliomyelitis, with potentially fatal consequences~\citep{Attwell2021}. 
% \EB{Citation if you want one: Attwell, K., Smith, D. T., and Ward, P. R. (2021). ‘“If your child's vaccinated, why do you care about mine?” Rhetoric, responsibility, power and vaccine rejection', Journal of Sociology 57(2): 268-285. https://doi.org/10.1177/1440783319893468 and Evelyn, K. (2020). ‘Advocates blame anti-vaxxers after four-year-old boy dies from flu', The Guardian, 3 August, URL (consulted 3 August 2023): https://www.theguardian.com/us-news/2020/feb/07/colorado-boy-dies-flu-anti-vaccine-facebook-groups .}
The reach and consequences of misinformation are amplified by the increasing use of online social media as a primary source of news and information~\cite{Shearer:2021vb}.
For example, \citet{kydd2021decline} blames social media for mainstreaming conspiracy theorizing, resulting in the attack on the US Capitol by devout QAnon followers. 
Due to the diverse range of ways misinformation can influence believers, it follows that misinformation cannot be studied in isolation. 
It is crucial to consider what is being shared in context: who is sharing it, who are the likely consumers and how it is being shared to reach the audiences effectively.
%In this work, we study the misinformation ecosystem in Australia; 
%we propose that misinformation is created and consumed as an online product targeted to specific vulnerable populations.
In this work, we examine how far-right and fringe online groups share and leverage news media articles to advance their narratives, to understand the role of news publishers in potentially unintentionally propagating misinformation. 
% \EB{Since we're emphasising how people use the sources to their own ends, we want to emphasise that (at least some) news publishers are publishing without the intention to fuel conspiracy etc.} MAR: OK.
% we qualitatively define the personas of populations vulnerable to misinformation

%The growing impacts of misinformation has been exacerbated by the increasing percentage of the population relying on social media for news and information~\cite{Shearer:2021vb}. The exposure and reactions to misinformation differ by countries and they experience different aspects of misinformation~\cite{kaur2018information, knuutila2022afraid}.
%\TODO{MAR}{The intro reads a lot nicer, but I lack one thing: it does not talk about the news environment at all, and RQ1 drops out of nowhere.}
% The consequences of misinformation have been amplified by the increasing proportion of the population turning to social media as a primary source of news and information~\cite{Shearer:2021vb}. 
% For example, \citet{kydd2021decline} suggests that the rise of social media leads to the mainstreaming of conspiracy theorizing, resulting in the attack on the US Capitol. 
% %\EB{Do you want to give examples of the consequences? I have some citations if so but things like the attack on the Capitol in the US in 2021, or loss of herd immunity to old illnesses from vaccine misinformation could work.} 
% %\st{The dissemination and responses to misinformation exhibit variations across different countries, leading to distinct experiences with regard to its multifaceted manifestations} \mar{This is a mouthful! What does this mean?}
% %On the other hand, the role of traditional news media was perceived as providing evidence-based information to the general public~\cite{zarocostas2020fight}. Recently, however, since traditional news is mostly consumed via online social media, who is sharing and how it is shared became more crucial than what is being shared to reach audience. In this paper, we study Australian news media in order to understand the role of mainstream news publishers in creating/spreading misinformation. Furthermore, we investigate news articles that are shared by far-right social media users to assess indications of misinformation.  
% On the other hand, traditional news media have long been perceived as providers of evidence-based information to the general public~\cite{zarocostas2020fight}. 
% However, in recent times, with the predominant consumption of traditional news occurring through online social media platforms, the focus has shifted. 
% It has become increasingly crucial to consider what is being shared, who is sharing it, and how it is being shared to reach the audience effectively. 
% In this paper, our study centers on Australian news media to gain insight into the role of mainstream news publishers in disseminating and potentially propagating misinformation. 
% Furthermore, we investigate news articles shared by users from far-right social media circles to identify any indications of misinformation.

%How misinformation spreads varies depending on the country, and this study focuses on that Australian context~\cite{kaur2018information, knuutila2022afraid}.
%the motivation for this sentence is to emphasize that we are studying Australian misinformation specifically 

%To study three of the vulnerable cohorts, we build archetypal personas of misinformation consumers in Australia and observe that each cohort represented by this persona has a preferred writing style and delivery format.
%Therefore, we delve deeper into quantifying their communication styling.
%We show, using real-world experiments using styled Facebook ads, that communication effectiveness is significantly boosted by applying styling adapted to the recipient's taste.

% In response to the prevalence of online abusive and misinformational content that eluded detection and repercussions, online platforms implemented countermeasures such as independent fact-checking social media posts. 
% However, these measures faced challenges as determined users began employing alternative tactics, such as avoiding specific terms and overloading the meaning of others to evade censorship. 
% Therefore, our research endeavors to explore text style inherently more resistant to manipulation than its content, given the evolving landscape of online content and user behavior~\cite{da2022text}.\mar{@EB: can we have a one-sentence definition of text style? or simply an explanation of what it is.}
% %\mar{Is that what we're doing?\EB{I thought maybe we were looking at styles that were more vulnerable to manipulation.}} 

\begin{figure}[tbp]
\includegraphics[scale=0.32]{imgs/flow.pdf}
\centering
\caption{Summary of the methods: we start by analysing contents of Australian news articles and sharing patterns of those articles in Twitter environment. Then we use linguistic styles captured by \textsc{LIWC}, \textsc{Grievance} dictionary and \textsc{StyloMetrix}, instead of contents, to identify extreme groups in Facebook. Next, we identify text styles employed by the extreme groups and classify them. Finally, we distinguish misinformation production and consumption using styles.}
\label{fig:introduction}
\end{figure}
% 4 step strategy:
%In this study, we first analyze the landscape of Australian News media consumption by comparing news articles from different ideological groups and also comparing news articles shared by extreme partisan online users. This step is to see if there are content wise distinctions in the extreme groups. Then, we use style related features, without looking at contents, to distinguish extreme ideological groups. We observe that we can differentiate the groups using only stylistic features as well as content based methods. Based on the observations, we attempt to detect our hand labeled styles in  the texts from the extreme groups. Finally, we test our hypothesis in the wild by deploying real-world advertisements to compare reactions on styled, not styled and wrongly styled texts. 
%\mar{It is weird to have the summary of work \& contributions before outlining the research questions.} \EB{I think this overview could be cut or considerably trimmed if you need space--don't the research questions and list of contributions give an overview?}


%To better understand dynamics of misinformation in Australian  
%We analyzed the landscape of Australian News media consumption and observed few difference among ideological groups in their misinformational news consumption patterns. In addition, there was no noticeable linguistic differences among news articles from different publishers. 


%Motivated by our observations, we hypothesize that misinformation is a process of misinformation consumption pattern. In other words, we treat misinformation consumption pattern as a pathway that connects consumers to creators using a distinct packaging of misinformation. 
%Without diving into definitions, actors, characteristics
% observation, detection and intervention
%we suggest that awareness of, exposure to, and reactions to misinformation are best understood in terms of social media use and left–right ideology.
%Unlike some previous research outputs, we found that the relations

% show the misinformation ecosystem figure here

\textbf{Research Questions:} 
In this paper, we use content- and style-based measures to show that misinformation, like any other content, can be styled to target particular online cohorts. Together, these elements and their users make up a misinformation ecosystem.
In particular, we answer the following research questions (RQs):
\begin{itemize}
    \item \textbf{RQ1:} \textit{What role do the style and content of news media play in enabling the spread of misinformation?}%\mar{@JL: I quite like leading with this RQ concerning the news media. Can we add it?}
    %\item \textbf{RQ2:} {\it How is misinformation packaged within the Australian online media, and which demographics are particularly susceptible?}
    %{\it How is misinformation packaged to reach consumers?}
    % Ask Emily for social science theory papers
    \item \textbf{RQ2} %{\it Can we differentiate between texts originating from distinct extremist groups using linguistic styles?}
    {\it Can we differentiate fringe groups based on linguistic styles?}
    %\item \textbf{RQ4:} %{\it Do styled texts demonstrate greater effectiveness in conveying messages?}
    \item \textbf{RQ3}
    {\it Can we differentiate contents from producers and consumers based on linguistic styles? }
    %{\it Do messages styled for distinct fringe groups demonstrate greater effectiveness in eliciting a response from the cohort?}
\end{itemize}
%\revEB{Suggested RQ1: What role do the style and/or content of Australian news media play in enabling the spread of misinformation? (Answer: it's not their content or style, but how users selectively share them) RQ2: Can we differentiate fringe groups based on linguistic styles? (Answer: Yes) RQ3: Do messages styled for distinct fringe groups demonstrate greater effectiveness in eliciting a response from the cohort? (Answer: yes)}

Our contributions are as follows: 
\begin{enumerate}
    \item We provide an analysis that comparatively examines the ideological landscape of Australian news and how users selectively share news to further their own ends regardless of the source ({\bf RQ1}).
    % \EB{Adding back in the cool finding that keeps getting buried!}
    %\item We present the concept of the misinformation ecosystem and formulate personas representing consumers of misinformation ({\bf RQ2}).
    \item We propose a classifier to identify linguistic styles within extreme online groups as well as styles that are commonly used in the online misinformation space. ({\bf RQ2}).
    %\item We conduct real-world experiments to assess the impact of styled texts on the demographics represented by our personas. ({\bf RQ4}).
    \item We show that production and consumption of misinformation exhibit different patterns that can be differentiated by styles ({\bf RQ3}).
\end{enumerate}
\cref{fig:introduction} depicts the steps of our analysis, the used datasets and methods.
\textcolor{blue}{In~\cref{}We start by analysing integrity of news articles with respect to their political ideology. }
We expand details of our contributions below. 

\subsubsection{Landscape of Australian news (\cref{sec:newsmedia})}
Starting from the assumption that misinformation is an information production problem, much of the prior work has studied the connection between misinformation, and the publishers' political leaning~\cite{calvillo2020political,das2022rethinking}. %stein2023network
% In order to investigate the significance of the language styles of extreme online users as distinct from the topics they discuss, 
%We perform a comprehensive analysis of Australian news media consumption. Using the Trust Index (a measure of information completeness), we compare news articles from legacy news media publishers with distinct ideological stances. We also look for writing style differences. Additionally, we analyze the sharing patterns of news articles by highly partisan online users. Our analysis identifies some content-based differentiations among news sources and extreme ideological cohorts. We discover that there are noticeable differences when we compare articles shared by extreme online users with articles published by far-right news media in terms of linguistic patterns. It is interesting since we find less distinction between far-right and moderate articles. Even for the few significant differences, we find small effect sizes indicating that the sharing of extreme content is less related to the source's reliability and more about how users interpret and exploit a source. This leads us to conclude that misinformation is less of an information production problem. We next investigate if it is an information consumption problem.
We conducted a comprehensive analysis of Australian news media consumption, focusing on several key aspects. Firstly, we utilized the Trust Index, a metric measuring information completeness, to compare news articles from legacy news media publishers with distinct ideological stances. Secondly, we examined writing style differences across these sources. Additionally, we delved into the sharing patterns of news articles by highly partisan online users.

Our analysis revealed content-based differentiations among news sources and extreme ideological cohorts. Interestingly, we observed significant differences when comparing articles shared by extreme online users with articles published by far-right news media, particularly in terms of linguistic patterns. Notably, we found less distinction between far-right and moderate articles. Even in cases where differences were statistically significant, the effect sizes were small, indicating that the sharing of extreme content is less tied to the source's reliability and more about how users interpret and leverage a source.

This leads us to the conclusion that misinformation may be less of an issue related to information production and more of an issue tied to information consumption. To explore this further, we investigate whether it is an information consumption problem.

%\subsubsection{Misinformation Ecosystem and Personas (\cref{misinfo_ecosystem} and \cref{sec:advertisements})}
%Through qualitative analysis of fringe and extreme online communities, we observe that certain groups of misinformation consumers exhibit heightened susceptibility to particular styling of misinformation -- for example, an intimate writing style in a ``junk science'' reporting format.
%We propose a misinformation ecosystem in which vulnerable consumers consume content of particular styling produced by dedicated misinformation creators.
% which shows pathways of vulnerable consumers as an adoption of the packaging. 
%We also develop representative vulnerable personas, which we use to guide a real-world experiment using Facebook advertisements.  
%This study uses stylistic metrics from established dictionaries to construct a classifier for discerning text sources. 
%Additionally, we classify styles labeled by human annotators using these stylistic measures.
%Then, we employ stylistic measures, without recourse to the article contents, to separate the extreme ideological factions. 

\subsubsection{Classification of Extreme Online Groups and Styles (\cref{styleovercontent})}
This study uses stylistic metrics from established dictionaries (such as \textsc{LIWC} and the \textsc{Grievance} dictionary) to construct stylistic classifiers.
% for discerning text sources.
Using these stylistic classifiers, we can accurately distinguish vulnerable misinformation consumers (like anti-vaccination and far-right) from regular online social media users (\cref{subsec:misleadingstyles}).
% From the classification results, we discover that the differentiation of groups based solely on stylistic attributes is as good as content-based classifiers. %\EB{I am unsure what this sentence is about, as it currently reads like the stylistic attributes are drawn form the news article analysis.} 
We further show that we can detect extreme ideological users' writing styles, as categorized by our manual labeling (\cref{subsec:identify-styles}). 
Lastly, we show that we can successfully distinguish far-right sources from far-right consumers using a stylistic classifier (\cref{pro_con_classify}).
%Lastly, based on the finding that the news articles published by far-right sources significantly differ from the articles shared by far-right Twitter users, we build a style-based classifier and distinguish them (\cref{pro_con_classify}). 
%\subsubsection{Real-world experiments (\cref{sec:advertisements})}
%Finally, we perform a real-world experiment, comparing the effectiveness of Facebook ads that have been styled, unstyled, and incorrectly styled for their target demographic. 
%We find that styled messages are significantly more effective in communicating with the target online demographics.
%% The analysis of user reactions in the live environment validates our hypotheses. 
%This sheds light on the broader implications of styled texts in the context of both misinformation and news media consumption. 

% \cref{fig:introduction} depicts the steps of our analysis, the used datasets and methods. 
% Our analysis points to two key findings: 
% 1) text styles from extreme online communities can be detected using style-based metrics, and 
% 2) styled messages are more effective in communicating with online demographics.

%\hl{The structure of this paper is as follows:  We begin by surveying measures on misinformation detection and intervention. We then present misinformation consumption patterns in Australian news articles. Next, we build a style-based classifier to distinguish the two extreme online groups and to detect styles in texts from the groups. We lastly test our proposed misinformation ecosystem by employing styled texts in the wild.}\mar{I always thought such ``paper structure'' paragraphs were obsolete and useless.}



==> sections/sec1-intro.tex <==
\section{Introduction}
\label{sec:introduction}

%\revEB{Test writing from Emily}
%\EB{Comment from Emily.}
\begin{comment}
\verify{
    I suggest the following changes to the structure:
    \begin{itemize}
        \item Sec 2: section of ``Datasets \& Prerequisites'' (Google News -- remove TDE name --, Twitter far right, Facebook antivax and Facebook far-right) and measures of content (Trust Index) and style (LIWC, StyloMetrix, Grievances)
        \item Sec 3 (or 4): We start by showing there is very little difference between the news articles published by publishers of different political leaning (including far-right). We measure the completeness of the information and even the style. We look at articles produced by publishers considered far-right and those shared by far-right Twitter users. Almost as if the problem is not in the information itself.
        \item Sec 4 (or 3): our main contribution: misinformation and problematic content is an eco-system + styling + personas + qualitative experiment Need here:
        \begin{itemize}
            \item the cards of the personas (maybe in SI)
            \item bring together the identification of style and identification of groups in this order. We need tables of results.
            \item statistical testing results on ads experiment? See \url{https://towardsdatascience.com/a-b-testing-a-complete-guide-to-statistical-testing-e3f1db140499}, section "Discreete metrics"
        \end{itemize}
        \item sec 5: Related work
        \item Sec 6: conclusion
    \end{itemize}
}
\end{comment}
%The growing impacts of misinformation has been exacerbated by the increasing percentage of the population relying on social media for news and information~\cite{Shearer:2021vb}. The exposure and reactions to misinformation differ by countries and they experience different aspects of misinformation~\cite{kaur2018information, knuutila2022afraid}.
%\TODO{MAR}{The intro reads a lot nicer, but I lack one thing: it does not talk about the news environment at all, and RQ1 drops out of nowhere.}
The consequences of misinformation have been amplified by the increasing proportion of the population turning to social media as a primary source of news and information~\cite{Shearer:2021vb}. 
For example, \citet{kydd2021decline} suggests that the rise of social media leads to the mainstreaming of conspiracy theorizing, resulting in the attack on the US Capitol. 
%\EB{Do you want to give examples of the consequences? I have some citations if so but things like the attack on the Capitol in the US in 2021, or loss of herd immunity to old illnesses from vaccine misinformation could work.} 
%\st{The dissemination and responses to misinformation exhibit variations across different countries, leading to distinct experiences with regard to its multifaceted manifestations} \mar{This is a mouthful! What does this mean?}
%On the other hand, the role of traditional news media was perceived as providing evidence-based information to the general public~\cite{zarocostas2020fight}. Recently, however, since traditional news is mostly consumed via online social media, who is sharing and how it is shared became more crucial than what is being shared to reach audience. In this paper, we study Australian news media in order to understand the role of mainstream news publishers in creating/spreading misinformation. Furthermore, we investigate news articles that are shared by far-right social media users to assess indications of misinformation.  
On the other hand, traditional news media have long been perceived as providers of evidence-based information to the general public~\cite{zarocostas2020fight}. 
However, in recent times, with the predominant consumption of traditional news occurring through online social media platforms, the focus has shifted. 
It has become increasingly crucial to consider what is being shared, who is sharing it, and how it is being shared to reach the audience effectively. 
In this paper, our study centers on Australian news media to gain insight into the role of mainstream news publishers in disseminating and potentially propagating misinformation. 
Furthermore, we investigate news articles shared by users from far-right social media circles to identify any indications of misinformation.

%How misinformation spreads varies depending on the country, and this study focuses on that Australian context~\cite{kaur2018information, knuutila2022afraid}.
%the motivation for this sentence is to emphasize that we are studying Australian misinformation specifically 

In response to the prevalence of online abusive and misinformational content that eluded detection and repercussions, online platforms implemented countermeasures such as independent fact-checking social media posts. 
However, these measures faced challenges as determined users began employing alternative tactics, such as avoiding specific terms and overloading the meaning of others to evade censorship. 
Therefore, our research endeavors to explore text style inherently more resistant to manipulation than its content, given the evolving landscape of online content and user behavior~\cite{da2022text}.\mar{@EB: can we have a one-sentence definition of text style? or simply an explanation of what it is.}
%\mar{Is that what we're doing?\EB{I thought maybe we were looking at styles that were more vulnerable to manipulation.}} 

\begin{figure}[tbp]
\includegraphics[scale=0.33]{imgs/intro_new.pdf}
\centering
\caption{Summary of the methods.}
\label{fig:introduction}
\end{figure}

% 4 step strategy:
%In this study, we first analyze the landscape of Australian News media consumption by comparing news articles from different ideological groups and also comparing news articles shared by extreme partisan online users. This step is to see if there are content wise distinctions in the extreme groups. Then, we use style related features, without looking at contents, to distinguish extreme ideological groups. We observe that we can differentiate the groups using only stylistic features as well as content based methods. Based on the observations, we attempt to detect our hand labeled styles in  the texts from the extreme groups. Finally, we test our hypothesis in the wild by deploying real-world advertisements to compare reactions on styled, not styled and wrongly styled texts. 
%\mar{It is weird to have the summary of work \& contributions before outlining the research questions.} \EB{I think this overview could be cut or considerably trimmed if you need space--don't the research questions and list of contributions give an overview?}


%To better understand dynamics of misinformation in Australian  
%We analyzed the landscape of Australian News media consumption and observed few difference among ideological groups in their misinformational news consumption patterns. In addition, there was no noticeable linguistic differences among news articles from different publishers. 


%Motivated by our observations, we hypothesize that misinformation is a process of misinformation consumption pattern. In other words, we treat misinformation consumption pattern as a pathway that connects consumers to creators using a distinct packaging of misinformation. 
%Without diving into definitions, actors, characteristics
% observation, detection and intervention
%we suggest that awareness of, exposure to, and reactions to misinformation are best understood in terms of social media use and left–right ideology.
%Unlike some previous research outputs, we found that the relations

% show the misinformation ecosystem figure here

\textbf{Research Questions:} 
In this paper, we use content- and style-based measures to show that misinformation, like any other content, can be styled to target particular online cohorts, and together, these elements make up a misinformation ecosystem.
In particular, we answer the following research questions (RQs):
\begin{itemize}
    \item \textbf{RQ1:} \textit{What role do the style and content of Australian news media play in enabling the spread of misinformation?}%\mar{@JL: I quite like leading with this RQ concerning the news media. Can we add it?}
    \item \textbf{RQ2:} {\it How is misinformation packaged within the Australian online media, and which demographics are particularly susceptible?}
    %{\it How is misinformation packaged to reach consumers?}
    % Ask Emily for social science theory papers
    \item \textbf{RQ3:} %{\it Can we differentiate between texts originating from distinct extremist groups using linguistic styles?}
    {\it Can we differentiate fringe groups based on linguistic styles?}
    \item \textbf{RQ4:} %{\it Do styled texts demonstrate greater effectiveness in conveying messages?}
    {\it Do messages styled for distinct fringe groups demonstrate greater effectiveness in eliciting a response from the cohort?}
\end{itemize}
%\revEB{Suggested RQ1: What role do the style and/or content of Australian news media play in enabling the spread of misinformation? (Answer: it's not their content or style, but how users selectively share them) RQ2: Can we differentiate fringe groups based on linguistic styles? (Answer: Yes) RQ3: Do messages styled for distinct fringe groups demonstrate greater effectiveness in eliciting a response from the cohort? (Answer: yes)}

Our contributions are as follows: 
\begin{enumerate}
    \item We provide an analysis that comparatively examines the ideological landscape of Australian news ({\bf RQ1}).
    \item We present the concept of the misinformation ecosystem and formulate personas representing consumers of misinformation ({\bf RQ2}).
    \item We propose a classifier to identify linguistic styles within extreme online groups. ({\bf RQ3}).
    \item We conduct real-world experiments to assess the impact of styled texts on the demographics represented by our personas. ({\bf RQ4}).
\end{enumerate}
We expand on each of contributions below. 
\subsubsection{Landscape of Australian news (\cref{sec:newsmedia})}
Starting from the assumption that misinformation is an information production problem, much of the prior work has studied the connection between misinformation, and the publishers' political leaning~\cite{calvillo2020political,das2022rethinking,stein2023network}.
% In order to investigate the significance of the language styles of extreme online users as distinct from the topics they discuss, 
We perform a comprehensive analysis of Australian news media consumption. 
Using the Trust Index (a measure of information completeness), we compare news articles from legacy news media publishers with distinct ideological stances.
We also look for writing style differences.
Furthermore, we also analyze the sharing patterns of news articles by highly partisan online users. 
Our analysis identifies some content-based differentiations among news sources and extreme ideological cohorts.
But even for the few significant differences, we find small effect sizes.
This leads us to conclude that misinformation is not as much an information production problem.
We next investigate if it is an information consumption problem.

\subsubsection{Misinformation Ecosystem and Personas (\cref{misinfo_ecosystem} and \cref{sec:advertisements})}
Through qualitative analysis of fringe and extreme online communities, we observe that certain groups of misinformation consumers exhibit heightened susceptibility to particular styling of misinformation -- for example, an intimate writing style in a ``junk science'' reporting format.
We propose there exists a misinformation ecosystem in which vulnerable consumers consume content of particular styling produced by dedicated misinformation creators.
% which shows pathways of vulnerable consumers as an adoption of the packaging. 
We also develop representative vulnerable personas, which we use in a real-world experiment using Facebook advertisements.  
%This study uses stylistic metrics from established dictionaries to construct a classifier for discerning text sources. 
%Additionally, we classify styles labeled by human annotators using these stylistic measures.
%Then, we employ stylistic measures, without recourse to the article contents, to separate the extreme ideological factions. 

\subsubsection{Classification of Extreme Online Groups and Styles (\cref{subsec:misleadingstyles})}
This study uses stylistic metrics from established dictionaries (such as LIWC and the Grievances dictionary) to construct stylistic classifiers.
% for discerning text sources.
We show that using these stylistic classifiers we can accurately distinguish between vulnerable misinformation consumers (like anti-vaccination and far-right) from regular online social media users.
% From the classification results, we discover that the differentiation of groups based solely on stylistic attributes is as good as content-based classifiers. %\EB{I am unsure what this sentence is about, as it currently reads like the stylistic attributes are drawn form the news article analysis.} 
We further show that we can detect among the writing styles of users from extreme ideological groups, as categorized by our manual labeling. 

\subsubsection{Real-world experiments (\cref{sec:advertisements})}
Finally, we execute real-world advertisements, comparing the reactions to texts that have been styled, unstyled, and incorrectly styled for their target demographic. 
The analysis of user reactions in the live environment validates our hypotheses and sheds light on the broader implications of styled texts in the context of both misinformation and news media consumption. 

Taken all together, the overall process is depicted in \cref{fig:introduction}. 
Our analysis points to two key findings: 1) text styles from extreme online communities can be detected using style-based metrics, and 2) styled messages are more effective in communicating with online demographics.

%\hl{The structure of this paper is as follows:  We begin by surveying measures on misinformation detection and intervention. We then present misinformation consumption patterns in Australian news articles. Next, we build a style-based classifier to distinguish the two extreme online groups and to detect styles in texts from the groups. We lastly test our proposed misinformation ecosystem by employing styled texts in the wild.}\mar{I always thought such ``paper structure'' paragraphs were obsolete and useless.}


